Distilling the Undistillable: Learning from a Nasty Teacher

The inadvertent stealing of private/sensitive information using Knowledge Distillation (KD) has been getting significant attention recently and has guided subsequent defense efforts considering its critical nature. Recent work Nasty Teacher proposed to develop teachers which can not be distilled or imitated by models attacking it. However, the promise of confidentiality offered by a nasty teacher is not well studied, and as a further step to strengthen against such loopholes, we attempt to bypass its defense and steal (or extract) information in its presence successfully. Specifically, we analyze Nasty Teacher from two different directions and subsequently leverage them carefully to develop simple yet efficient methodologies, named as HTC and SCM, which increase the learning from Nasty Teacher by upto 68.63% on standard datasets. Additionally, we also explore an improvised defense method based on our insights of stealing. Our detailed set of experiments and ablations on diverse models/settings demonstrate the efficacy of our approach.

==> background.tex <==
% \section{Preliminaries}
% \label{sec:preliminaries}
\section{Method}
\subsection{Background: Knowledge Distillation}
\label{background:kd}
\noindent An ordinary training of Neural Network involves matching the output logits of a network $z$ with the truth label $y$, using the Cross-Entropy loss function. 
\begin{equation}
\label{eq:orig-ce-loss}
\mathcal{L}_{CE} = H(softmax(z), y)
\end{equation}
% \textcolor{magenta}{Arghya's comment: Merge the paragraph "Knowledge distillation ..." and "Formally, given ..." into one. It looks good when we describe using mathematical notations, i.e. the second paragraph,. Present version is describing and then again formally describing. "Knowledge distillation ..." paragraph seems redundant.}

\noindent In Knowledge distillation, a smaller Student Network ($f_s$) is trained with the output of a large Pre-Trained Teacher Network ($f_t$) alongside the ground-truth labels. Formally, with input image as $x$, and the output logits of student and teacher as $z_s= f_s(x)$  and $z_t= f_t(x)$ respectively, the logits are first softened using temperature $(\tau)$, transformed with softmax to obtain outputs $y_s$ and $y_t$:
\begin{equation}
    y_{s} = \textit{softmax}(z_{s}/\tau), 
    y_{t} = \textit{softmax}(z_{t}/\tau)
\end{equation}
and then passed through Kullback-Leibler(KL) divergence balanced by weight parameter $\lambda$ (generally $\lambda=\tau^{2}$ for KD) to compute KD loss as:
\begin{equation}
    \label{eq:orig-kd-loss}
    \mathcal{L}_{KD} = \lambda \cdot KL(y_s, y_t)
\end{equation}
% \textcolor{magenta}{Arghya's comment: Pls, check Eqn. \ref{eq:orig-kd-loss}. T or $\tau$?}
% Here, KL refers to the Kullback-Leibler Divergence and 
The final loss is now computed by combining $\mathcal{L}_{KD}$ with Eq. \ref{eq:orig-ce-loss} via parameter $\alpha$:
\begin{equation}
    \mathcal{L} = \alpha \cdot \mathcal{L}_{KD} + (1 - \alpha) \cdot \mathcal{L}_{CE}
    \label{eq:hinton-loss}
\end{equation}
% Here, $\alpha$ is the weight balancing parameter combining the individual objectives respectively.

% The equation \ref{eq:orig-kd-loss}, proposed by \cite{hinton} was
% \begin{equation}
%     \mathcal{L}_{KD} = \alpha KL(y_s / T, y_t / T) \times T^2

\begin{figure}[h]
    \centering
    % \includegraphics[page=1,width=0.75\linewidth]{imgs/ens/0.jpg}
%     \includegraphics[width=\linewidth]{imgs/ens/ens1.jpg}
%     \includegraphics[width=\linewidth]{imgs/ens/ens2.jpg}
%     \includegraphics[width=\linewidth]{imgs/ens/ens3.jpg}
	\includegraphics[width=\linewidth]{./imgs/ensv3.jpg}
    \caption{Probabilities of Nasty Teacher (a), Seq-1(b), Seq-2(c), their Ensemble(d) as used in \ensmeth, and Normal Teacher(e). As can be seen, probability distribution of Ensemble is very similar to Normal-Teacher. Note, Seq-i is $S^{i}$, Target Class is colored maroon and the remaining classes are colored orange.}
    \label{fig:nasty_illustration}
    % \vspace{-10pt}
\end{figure} 

\begin{figure}
    % \resizebox{2cm}{!}
    \centering
    % \includegraphics[width=\linewidth]{imgs/highT/tempmeth_yellow.jpg}
    
    
    \begin{tabular}{cc}
        % \includegraphics[width=0.45\linewidth]{imgs/highT/uniformity_brown.jpg}
        % & 
        % \includegraphics[width=0.5\linewidth]{imgs/tempmeth.jpg}
        \includegraphics[width=\linewidth]{./imgs/tempmeth_logits_horizontal.png}
        \\

    \end{tabular}
    \caption{The effect of temperature in HTC. We demonstrate the logits and probabilities at low temperature (as generally used in KD) and high temperature (as used in HTC). \textbf{(a)} Logits at low temperature $T_{low} = 4$, \textbf{(b)} Logits at high temperature $T_{high} = 50$, \textbf{(c)} Probabilities at $T_{low}$ , \textbf{(d)} Probabilities at $T_{high}$, \textbf{(e)} Composing with one-hot to increase the peak.}
    \label{fig:tempmeth-vis}
     \vspace*{-4mm}
\end{figure}

\subsection{Definition: KD Based Model Stealing}
% \textcolor{magenta}{Arghya's comment: Can we directly give Section name as "IP stealing"? instead of the Knowledge leakage ..?}
\noindent\underline{\textbf{KD-based Stealing}: }Given a stealer (or student) model $\theta_{st}$ and a victim (or teacher) $\theta_{vi}$, the stealer is said to succeed in stealing knowledge using KD if by using input-output information of victim it is able to grasp some additional knowledge which in the absence of teacher it won't have access to. Just like \cite{nasty}, we also think this phenomenon in terms of Maximum Accuracy of stealer with and without stealing from victim. Formally, considering the maximum accuracy of stealer model with and without stealing as $Acc_{w}(KD(\theta_{st}, \theta_{vi}))$ and $Acc_{wo}(\theta_{st})$, the stealing is said to happen if\\
\begin{equation}
    Acc_{w}(KD(\theta_{st}, \theta_{vi})) > Acc_{wo}(\theta_{st})
\end{equation}
Intuitively, the accuracy gain of stealer in the presence of victim (or teacher) indicates the additional beneficial information it was able to consume from the victim, thus the stealing. The aforementioned settings are same as used in \cite{nasty}, and we further discuss in \ref{ablations}. \\
% \subsection{Nasty Teacher: Defense for Knowledge Leaking}
\underline{\textbf{Defense against KD based Stealing}: } Following \cite{nasty}, we consider a method $M$ as defense, if it degrades the student's tendency (or accuracy) of stealing. Formally, considering the accuracy of stealer without defense $M$ as $Acc_{w}(KD((\theta_{st},\theta_{vi}))$ and with defense as $Acc_{wm}(KD(M(\theta_{st}, \theta_{vi})))$, $ M $ is said to be a defense if:
\begin{equation}
   Acc_{wm}(KD(M(\theta_{st},\theta_{vi}))) <  Acc_{w}(KD(\theta_{st},\theta_{vi})) 
\end{equation}
% Discussed earlier, the defense against Knowledge Distillation based stealing in a broader sense would either focus on revealing less number of output scores (e.g only top-K) or focus on obfuscating scores to make understanding them or inferring from them hard. 
In the next course of our discussion, we discuss Nasty Teacher \cite{nasty} following which we motivate our approach.

% write few lines on effective defense
% \textit{\textbf{Attack against such Defense}}: Now with defense $M$ applied to prevent any such leakage via KD, we define a method $A$ as an attack to defense $M$, if $A$ is able to increase the student's tendency of stealing from teacher. Formally, consider the accuracy of stealer in presence of defense $M$ without attack $A$ as $Acc_{wm}K(D((\theta_{st}, \theta_{vi}))$ and in presence of defense $M$ with attack $A$ as $Acc_{wa}(KD(A(M(\theta_{st}, \theta_{vi}))))$, $A$ is said to be an attack if:
% \begin{equation}
%   Acc_{wa}(KD(A(M(\theta_{st}, \theta_{vi})))) >  Acc_{wm}(KD((\theta_{st}, \theta_{vi}))
% \end{equation}
% The above accuracy gain thus signals the reduction of defense's efficacy and subsequent increase in extraction/leakage of information from teacher to student.\\
%write for the rest part of the paper here
